Direct bounds on Left-Right gauge boson masses at LHC Run 2

While the third run of the Large Hadron Collider (LHC) is ongoing, the underlying theory that extends the Standard Model remains so far unknown. Left-Right Models (LRMs) introduce a new gauge sector, and can restore parity symmetry at high enough energies. If LRMs are indeed realized in nature, the mediators of the new weak force can be searched for in colliders via their direct production. We recast existing experimental bounds from LHC Run 2 on the heavy LRM gauge boson masses. As a novelty, we discuss the effect of the LRM scalar content on the total width of the new gauge bosons, obtaining model-independent bounds within the specific realizations of the LRM scalar sectors analysed here. These bounds avoid the need to detail the spectrum of the scalar sector, and apply in the general case where no discrete symmetry is enforced. Moreover, we emphasize the effect of the structure of the quark right-handed mixing matrix on the charged LRM gauge boson production at LHC. We find that $W_R$ and $Z_R$ masses are constrained to lie above $2$ TeV and $4$ TeV, respectively.

==> table_summary.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|lc|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Channel} & \multirow{2}{*}{Refs.} & \multicolumn{2}{c|}{(i) $\Phi$ + $\chi_{L,R}$} & \multicolumn{2}{c|}{(ii) $\Phi$ + $\Delta_{L,R}$} & \multicolumn{2}{c|}{(iii) $\chi_{L,R}$} \\
        \cline{3-8}
         & & $M_{Z_R}$ & $M_{W_R}$ & $M_{Z_R}$ & $M_{W_R}$ & $M_{Z_R}$ & $M_{W_R}$ \\
        \hline
        \hline
        $Z_R \to \ell_i \bar{\ell}_i$ & \cite{CMS:2021ctt} & 4.3 & \rd{1.5} & 4.2 & \rd{1.0} & 4.3 & \rd{1.5}  \\
        %\hline
        %$Z_R \to j j$ & & & & & & & \\
        \hline
        \hline
        $W_R \to j j$, anti-diag. & \cite{ATLAS:2019fgd} & \rd{2.2} & 2.1 & \rd{3.0} & 2.0 & \rd{2.2} & 2.1 \\
        \hline
        $W_R \to \ell_i \bar{\nu}_R$, anti-diag. & \cite{ATLAS:2019lsy} & \rd{4.6} & 4.3 & \rd{6.3} & 4.2 & \rd{4.6} & 4.3 \\
        \hline
        \hline
        $W_R \to j j$, diag. & \cite{ATLAS:2019fgd} & \rd{3.1} & 2.9 & \rd{4.1} & 2.7 & \rd{3.2} & 3.0 \\
        \hline
        $W_R \to \ell_i \bar{\nu}_R$, diag. & \cite{ATLAS:2019lsy} & \rd{5.4} & 5.1 & \rd{7.5} & 5.0 & \rd{5.4} & 5.1 \\
        \hline
    \end{tabular}
    \caption{Summary of the bounds on the new gauge boson masses $ M_{Z_R} $ or $ M_{W_R} $, according to the case indicated in the first column. Two specific structures of the RH quark mixing matrix are considered, namely, a diagonal (i.e., CKM-like) and an anti-diagonal structures. The case $W_R \to \ell_i \bar{\nu}_R$ concerns light RH neutrinos. Bounds combine information from electronic and muonic modes. Values are given in TeV. [\rd{Numerical values in red should be re-discussed}]}
    \label{tab:summary_bounds}
    %[\rd{\textbf{problem giving only bounds from one source, if they are compatible?}: dijet is very similar (here we did the exercise a bit better), same for the other cases}]
    %[always smallest $g_R$?][Always light neutrino cases?]: the philosophy is establishing the lowest bounds; in $Z_R$ we take neutrinos to be accessible %[\rd{are we discussing heavy RH neutrinos somewhere?: no}]
    %\rd{[We have been employing the observed limits? Sergio: Yes]}
    %[\rd{include the top; correct acceptance in the $W_R \to j j$ case}]
    %THREE options: (1) calculating the bounds strictly by varying $\gamma$, (2) not displaying the conversion in the table above, (3) showing bounds as they are above, but rising red flags
\end{table}
